Multi-Task Multi-Scale Contrastive Knowledge Distillation for Efficient Medical Image Segmentation

This thesis aims to investigate the feasibility of knowledge transfer between neural networks for medical image segmentation tasks, specifically focusing on the transfer from a larger multi-task "Teacher" network to a smaller "Student" network. In the context of medical imaging, where the data volumes are often limited, leveraging knowledge from a larger pre-trained network could be useful. The primary objective is to enhance the performance of a smaller student model by incorporating knowledge representations acquired by a teacher model that adopts a multi-task pre-trained architecture trained on CT images, to a more resource-efficient student network, which can essentially be a smaller version of the same, trained on a mere 50% of the data than that of the teacher model. To facilitate knowledge transfer between the two models, we devised an architecture incorporating multi-scale feature distillation and supervised contrastive learning. Our study aims to improve the student model's performance by integrating knowledge representations from the teacher model. We investigate whether this approach is particularly effective in scenarios with limited computational resources and limited training data availability. To assess the impact of multi-scale feature distillation, we conducted extensive experiments. We also conducted a detailed ablation study to determine whether it is essential to distil knowledge at various scales, including low-level features from encoder layers, for effective knowledge transfer. In addition, we examine different losses in the knowledge distillation process to gain insights into their effects on overall performance.

==> 00_Intro_Pages/03a_Certificate.tex <==
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%	                                   CERTIFICATE A	                                  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
\begin{center}
{\large{\bf{\underline{CERTIFICATE}}}}
\end{center}
%\thispagestyle{empty}


\noindent
This is to certify that the Dissertation entitled \textbf{``Advancing Medical Image Segmentation Through Multi-Task and Multi-Scale Contrastive Knowledge Distillation''} and submitted by Mr. Risab Biswas, ID No.: 2021SC04063 in partial fulfillment of the requirements of DSECLZG628T Dissertation, embodies the work
done by him/her under my supervision.

\vspace{4cm}
\noindent
\textbf{Signature of the Supervisor} \hfill Name: Dr. Chaitanya Kaul \\
\noindent Place: University of Glasgow \hfill Designation: Research Associate \\
Date:  \noindent \today
% \noindent Thiruvananthapuram - 695 551 \hfill [Project Supervisor]
\begin{center}
 
\end{center}
\clearpage



==> 00_Intro_Pages/07_Abbrev,Const,Symbols.tex <==
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%                               NOTATIONS AND ABBREVIATIONS                               %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% NOTE: YOU WILL NEED TO ENABLE LINES 115-125 of report.tex OR
%       MAKE USE OF THE listsofsymbols PACKAGE

% The listof___ inputs below are used to generate tables for the symbols,
% constants and nomenclature and take inputs of l, c, r to determine their
% respective column alignments as do any other tables in  LaTeX.

\clearpage % Start a new page

\setstretch{1.5} % Set the line spacing to 1.5, this makes any following tables easier to read.

\noindent

{\Huge{\bf{Notations and Abbreviations}}}\
\\[6pt] 

% NOTE: YOU WILL NEED TO ENABLE LINES 127-137 of report.tex
% sAMPLE OF USE:

\listofsymbols{ll} % Include a list of Abbreviations (a table of two columns)
{
\textbf{FEA} & \textbf{F}inite \textbf{E}lement \textbf{A}nalysis \\
\textbf{FEM} & \textbf{F}inite \textbf{E}lement \textbf{M}ethod \\
\textbf{LVDT} & \textbf{L}inear \textbf{V}ariable \textbf{D}ifferential \textbf{T}ransformer \\
\textbf{RC} & \textbf{R}einforced \textbf{C}oncrete\\
\textbf{Acronym} & \textbf{W}hat (it) \textbf{S}tands \textbf{F}or \\
}


\newpage


==> Appendices/A_AppA.tex <==
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%                                    APPENDIX TEMPLATE                                    %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%

% Use these after the \appendix command at the end of report.tex
% Appendices work similar to a chapter and are used to provide supplementary information that typically do not contribute to the final page count of a report.

\chapter{Long Appendix Title Here} % Main appendix title

\label{AppendixA} % for referencing this appendix elsewhere, use \ref{AppendixA}

% This is for the header on each page if in use - input a shortened title due to constrictions.
% \lhead{Appendix A. \emph{Short App. Title Here}}

Write your Appendix content here. Sections and subsections can be used as well.
\section{First Appendix Section}
\subsection{First Appendix Subsection}
\subsubsection{First Appendix Subsubsection}
Appendices will show up in the ToC numbered as letters. This is of course totally customizable, please refer to the CTAN documentation (\url{https://ctan.org/pkg/appendix?lang=en}) for further clarity on the same.

==> Images/Figures/3D_Cone.tex <==
% 3D Cone
% Author: Gene Ressler. Adapted to TikZ by Kjell Magne Fauske.
% See http://www.frontiernet.net/~eugene.ressler/ for more details.

\begin{tikzpicture}[join=round, scale=2]
    \tikzstyle{conefill} = [fill=blue!20,fill opacity=0.8]
    \tikzstyle{ann} = [fill=white,font=\footnotesize,inner sep=1pt]
    \tikzstyle{ghostfill} = [fill=white]
         \tikzstyle{ghostdraw} = [draw=black!50]
    \filldraw[conefill](-.775,1.922)--(-1.162,.283)--(-.274,.5)
                        --(-.183,2.067)--cycle;
    \filldraw[conefill](-.183,2.067)--(-.274,.5)--(.775,.424)
                        --(.516,2.016)--cycle;
    \filldraw[conefill](.516,2.016)--(.775,.424)--(1.369,.1)
                        --(.913,1.8)--cycle;
    \filldraw[conefill](-.913,1.667)--(-1.369,-.1)--(-1.162,.283)
                        --(-.775,1.922)--cycle;
    \draw(1.461,.107)--(1.734,.127);
    \draw[arrows=<->](1.643,1.853)--(1.643,.12);
    \filldraw[conefill](.913,1.8)--(1.369,.1)--(1.162,-.283)
                        --(.775,1.545)--cycle;
    \draw[arrows=->,line width=.4pt](.274,-.5)--(0,0)--(0,2.86);
    \draw[arrows=-,line width=.4pt](0,0)--(-1.369,-.1);
    \draw[arrows=->,line width=.4pt](-1.369,-.1)--(-2.1,-.153);
    \filldraw[conefill](-.516,1.45)--(-.775,-.424)--(-1.369,-.1)
                        --(-.913,1.667)--cycle;
    \draw(-1.369,.073)--(-1.369,2.76);
    \draw(1.004,1.807)--(1.734,1.86);
    \filldraw[conefill](.775,1.545)--(1.162,-.283)--(.274,-.5)
                        --(.183,1.4)--cycle;
    \draw[arrows=<->](0,2.34)--(-.913,2.273);
    \draw(-.913,1.84)--(-.913,2.447);
    \draw[arrows=<->](0,2.687)--(-1.369,2.587);
    \filldraw[conefill](.183,1.4)--(.274,-.5)--(-.775,-.424)
                        --(-.516,1.45)--cycle;
    \draw[arrows=<-,line width=.4pt](.42,-.767)--(.274,-.5);
    \node[ann] at (-.456,2.307) {$r_0$};
    \node[ann] at (-.685,2.637) {$r_1$};
    \node[ann] at (1.643,.987) {$h$};
    \path (.42,-.767) node[below] {$x$}
        (0,2.86) node[above] {$y$}
        (-2.1,-.153) node[left] {$z$};
\end{tikzpicture}
